What Makes and Breaks Safety Fine-tuning? A Mechanistic Study

Safety fine-tuning helps align Large Language Models (LLMs) with human preferences for their safe deployment. To better understand the underlying factors that make models safe via safety fine-tuning, we design a synthetic data generation framework that captures salient aspects of an unsafe input by modeling the interaction between the task the model is asked to perform (e.g., "design") versus the specific concepts the task is asked to be performed upon (e.g., a "cycle" vs. a "bomb"). Using this, we investigate three well-known safety fine-tuning methods -- supervised safety fine-tuning, direct preference optimization, and unlearning -- and provide significant evidence demonstrating that these methods minimally transform MLP weights to specifically align unsafe inputs into its weights' null space. This yields a clustering of inputs based on whether the model deems them safe or not. Correspondingly, when an adversarial input (e.g., a jailbreak) is provided, its activations are closer to safer samples, leading to the model processing such an input as if it were safe. We validate our findings, wherever possible, on real-world models -- specifically, Llama-2 7B and Llama-3 8B.

==> Appendices/C.AnalyticalLipschitz.tex <==
\section{Analytical Analysis of Lipschitz Constant}
\label{sec:lips_analytical_analysis}
Consider a single layer pre-trained neural network ${f:~} \mathbb{R^{d}}\xrightarrow{}\mathbb{R^{k}}$ with weight ${W}$ ($\mathbb{R^{d\times k}}$), given by  ${{f}(x,y) = W^Tx}$, where ${k}$ is the number of classes. We consider the following assumptions:
\begin{itemize}
    \item \textbf{A1:} Let all the fine-tuning samples $x$ in the set {${P}$} = \safepr $\cup$ \unsafepr be orthonormal to each other ie. ${x_i^Tx_j=0}$ $\forall {i,j}; {i\neq j}$ and ${x_i^Tx_i=1}$.
    \item \textbf{A2:} Let the weights of the pre-trained model given by ${{W^T[c]=\Sigma_{i=1}^{n_c}\delta_ix_{i,c}}}$, where ${\delta_i}\geq0$, ${n_c}$ is the number of samples belonging to class ${c}$ and used for pre-training. Therefore, such a model gives perfect classification performance on samples used during pre-training.
    \item \textbf{A3:} Let the fine-tuning setting be defined as a single token prediction, where for unsafe samples, the model needs to predict the null token and for the safe samples, the model should predict any one of the remaining ${r-1}$ classes, where ${r}$ is the total number of classes. Let the class index corresponding to null token prediction be 1.
\end{itemize}

\subsection{Analysis of global lipschitzness}
The global lipschitzness constant of a function ${f}$ on a set $\mathcal{P}$ is defined as \citep{sanyal2019stable}:
\begin{equation}
\label{eq:lips}
   {L({f})} =  {max_{x_i, x_j} \frac{||{f}(x_i) - {f}({x_j})||_q}{||{x_i}-{x_j}||_p}}
\end{equation}
where, ${x_i}, {x_j}$ are any two different samples ie. ${i \neq j}$ drawn from $\mathcal{P}$. Let ${p=q=2}$.
Let the safety fine-tuning learning rate be given by $\alpha$ and the hyperparameter used in DPO  and unlearning be 1. For simplicity, in this analysis we use the same hyperparameter value for the positive and negative terms in DPO and unlearning. Thus we have
\begin{prop}
\label{prop:Unlearning} $\exists$ learning rate ${\alpha}$ where ${\alpha}<min({\delta_i})$, $\forall {i\leq n_c, \forall c\leq r}$  such that $\forall$ input samples  ${x} \in  \bgdbox{red}{$\mathcal{P_U}$}$, we have
${L({f_{\theta^{Unl}}})} \leq {L({f_{\theta^{SSFT}}})} \leq {L({f_{\theta^{IT}}})}$
\end{prop}
\begin{proof}
 Let ${x}$ be the input sample sampled from either \bgdbox{green}{$\mathcal{P_S}$} or  \bgdbox{red}{$\mathcal{P_U}$} and ${y_L}$, ${y_P}$ be the less preferred and more preferred output labels respectively. We denote ${\sigma[\log(e^{(W^Tx)_{{y_P}}})-\log(e^{(W^Tx)_{{y_L}}}]}$ as ${\gamma({x}, {y_L, y_P})}$.

% \textbf{Statement:} Given a single layer pre-trained neural network, optimizing the weights using DPO results in formation of clusters of safe and unsafe samples in the output space and also results in decreased value of the lipschitz constant for unsafe inputs.
The gradient with respect to weight ${W}$ for the DPO objective is given by:
\begin{equation}
    {\Delta_W L(x,y_L,y_P)} = -{\Sigma_{x,y_P,y_L}\sigma[\log(e^{(W^Tx)_{y_P}})-\log(e^{(W^Tx)_{y_L}}]}
    {[\Delta_W\log(e^{(W^Tx)_{y_P}})-\Delta_W\log(e^{(W^Tx)_{y_L}})]}
\end{equation}

\begin{equation}
    {\Delta_W L(x,y_L,y_P) = -\Sigma_{x,y_P,y_L}\gamma(x, y_P, y_L)([\mathbb{0,0,0},x,\mathbb{0},...]-[x,\mathbb{0,0,0},...])}
\end{equation}
where $\mathtt{[\mathbb{0,0,0},x,\mathbb{0},...]}$ is $\mathbb{R^{d\times k}}$
Therefore the gradient update for an unsafe sample $\mathtt{x_u} \in$ \bgdbox{red}{$\mathcal{P_U}$} is given by
\begin{equation}
\mathtt{W_t = W_{t-1} + [\alpha\gamma(x, y_P, y_L)x,\mathbb{0,0}.., \mathbb{0}] -[\mathbb{0}, ..., \mathbb{0}, \alpha\gamma(x, y_P, y_L)x, \mathbb{0},..., \mathbb{0}]}
\end{equation}
In case of $\mathtt{x_s} \in$ \bgdbox{green}{$\mathcal{P_S}$}, the gradient update is given by
\begin{equation}
\mathtt{W_t = W_{t-1} + [\mathbb{0}, ..., \mathbb{0}, \alpha\gamma(x, y_P, y_L)x, \mathbb{0},..., \mathbb{0}] - [\alpha\gamma(x, y_P, y_L)x, \mathbb{0}, \mathbb{0},.., \mathbb{0}]}
\end{equation}
Suppose the first p samples are unsafe and remaining t-p safe samples, then at time step t, the model will be given by
\begin{multline}
\label{eq:update}
    {W_t = W + \Sigma_{i=1}^p\alpha\gamma_ix_i[\mathbb{1},\mathbb{0,0,0,0},...] - \Sigma_{i=p+1}^t\alpha\gamma_ix_i[\mathbb{1},\mathbb{0,0,0,0},...]} - \\ {\Sigma_{i=1}^p\alpha\gamma_ix_i[\mathbb{0},\mathbb{1}(y_i==2),\mathbb{1}(y_i==3),..., \mathbb{1}(y_i==\mathbb{K})] +} \\ {\Sigma_{i=p+1}^t\alpha\gamma_ix_i[\mathbb{0},\mathbb{1}(y_i==2),\mathbb{1}(y_i==3),..., \mathbb{1}(y_i==\mathbb{K})]}
\end{multline}
where $\mathbb{1}, \mathbb{0} \in \mathbb{R^d}$ vectors with all rows having values 1 and 0 respectively.

If \bgdbox{green}{${x_i}$} and \bgdbox{green}{${x_j}$}, ${i \neq j}$ are safe samples, using the definition of global lipschitz constant in Eq~\ref{eq:lips} we get 
\begin{multline}
{{||f(\bgdbox{green}{$x_i$}) - f(\bgdbox{green}{$x_j$})||}=||W^T(\bgdbox{green}{$x_i$}-\bgdbox{green}{$x_j$}) + \alpha[(\gamma_j-\gamma_i)(\mathbb{1}, \mathbb{0,0}, ...)} - \\ {\gamma_j[\mathbb{0,0}, ...,\mathbb{1}, \mathbb{0}, ..., \mathbb{0}] + \gamma_i[\mathbb{0,0}, ...,\mathbb{1}, \mathbb{0}, ..., \mathbb{0}]||}
\end{multline}

If \bgdbox{red}{${x_i}$} and \bgdbox{red}{${x_j}$}, ${i \neq j}$ are unsafe, we get
\begin{multline}
{{||f(\bgdbox{red}{$x_i$}) - f(\bgdbox{red}{$x_j$})||}=||W^T(\bgdbox{red}{$x_i$}-\bgdbox{red}{$x_j$}) + \alpha[(\gamma_i-\gamma_j)(\mathbb{1}, \mathbb{0}, \mathbb{0}, ...)} - \\ {\gamma_i[\mathbb{0,0}, ...,\mathbb{1}, \mathbb{0}, ..., \mathbb{0}] + \gamma_j[\mathbb{0}, \mathbb{0}, ...,\mathbb{1}, \mathbb{0}, ..., \mathbb{0}]||}
\end{multline}
As discussed in {A2}, ${W[:,i]=\Sigma_{i=1}^l\delta_i x_{i, y_i}}$. This gives:
\begin{multline}
{{||f(\bgdbox{green}{$x_i$}) - f(\bgdbox{green}{$x_j$})||}=||\alpha(\gamma_j-\gamma_i)(\mathbb{1}, \mathbb{0,0}, ...)} - \\ {(\alpha\gamma_j+\delta_j)[\mathbb{0,0}, ...,\mathbb{1},  \mathbb{0}, ..., \mathbb{0}] + (\alpha\gamma_i+\delta_i)[\mathbb{0,0}, ...,\mathbb{1}, \mathbb{0}, ..., \mathbb{0}]||}
\end{multline}

\begin{multline}
{{||f(\bgdbox{red}{$x_i$}) - f(\bgdbox{red}{$x_j$})||}=||\alpha(\gamma_i-\gamma_j)(\mathbb{1}, \mathbb{0,0}, ...)} - \\ {(\alpha\gamma_i-\delta_i)[\mathbb{0,0}, ...,\mathbb{1}, \mathbb{0}, ..., \mathbb{0}] + (\alpha\gamma_j-\delta_j)[\mathbb{0,0}, ...,\mathbb{1}, \mathbb{0}, ..., \mathbb{0}]||}
\end{multline}
Thus maximum value is given by 
\begin{equation}
    {max_{x_i, x_j} {||f(\bgdbox{green}{$x_i$}) - f(\bgdbox{green}{$x_j$})||} =  max_{\gamma_i, \gamma_j,\delta_i, \delta_j}\sqrt{(\alpha(\gamma_i-\gamma_j))^2 + (\alpha\gamma_i+\delta_i)^2 + (\alpha\gamma_j+\delta_j)^2 }}
\end{equation}

\begin{equation}
    {max_{x_i, x_j} {||f(\bgdbox{red}{$x_i$}) - f(\bgdbox{red}{$x_j$})||} =  max_{\gamma_i, \gamma_j, \delta_i, \delta_j}\sqrt{(\alpha(\gamma_i-\gamma_j))^2 + (\alpha\gamma_i-\delta_i)^2 + (\alpha\gamma_j-\delta_j)^2 }}
\end{equation}
Therefore on using unsafe samples, the maximum value of lipschitzness constant can decrease for a suitable value of learning rate $\alpha$.

Further in case of unlearning, we have $\gamma_i=\gamma_j=1$, this gives:
\begin{equation}
        {max_{x_i, x_j} {||f(\bgdbox{red}{$x_i$}) - f(\bgdbox{red}{$x_j$})||} =   max_{\delta_i, \delta_j}\sqrt{(\alpha-\delta_i)^2 + (\alpha-\delta_j)^2 }}
\end{equation}
In case of supervised safety fine-tuning, this expression will be given by:
\begin{equation}
    {max_{x_i, x_j} {||f(\bgdbox{red}{$x_i$}) - f(\bgdbox{red}{$x_j$})||} =  max_{\delta_i, \delta_j}\sqrt{\alpha^2 + \delta_i^2 + (\alpha-\delta_j)^2 }}
\end{equation}
Thus we get
$\mathcal{L}(f_{\theta^{Unl}}) \leq \mathcal{L}({f_{\theta^{SSFT}}}) \leq \mathcal{L}({f_{\theta^{IT}}})$ for unsafe samples for some learning rate  $\alpha<\text{min}{\delta_j}$.

\end{proof}
On the other hand, for safe samples, we have $\mathcal{L}(f_{\theta^{Unl}}) \geq \mathcal{L}({f_{\theta^{SSFT}}}) \geq \mathcal{L}({f_{\theta^{IT}}})$. This is also observed in our empirical analysis about lipschitzness constant presented in the main paper.
% \subsection{Analysis of local lipschitzness}
% Here we have two additional assumptions, which are realistically feasible:
% \begin{itemize}
%     \item \textbf{A4:}  Since the model ${f}$ is not pre-trained to predict null token class which corresponds to the first output class, ${||W^T[0]||_2\approx 0}$.
%     \item \textbf{A5:}  ${||W^T[j]||} \approx {||W^T[k]||}$, $\forall$ ${j,k}$, where ${j} \neq {k}$ and ${j}, {k} \neq 0$.
    
% \end{itemize}
% Using these assumptions, we can prove that for an input sample ${x}\sim $\bgdbox{red}{$\mathcal{P_U}$}, the local lipschitzness of the model can decrease on using unlearning and DPO.
% \begin{proof}
    

% The local lipschitzness constant of a function ${f}$ for a sample ${x} \sim$ $\mathcal{P}$ is defined as \citep{sanyal2019stable}:
% \begin{equation}
% \label{eq:lips}
%    {L_{{x}}({f})} =  {\lim_{h\xrightarrow{}0} \frac{||{f}(x+h) - {f}({x})||_q}{||{h}||_p}} = {{||J_x({f})||_{p,q}}}
% \end{equation}
% where the Jacobian ${J_x(f)}$ is $\mathbb{R^{d\times K}}$ and is defined for the function ${f:~} \mathbb{R^{d}}\xrightarrow{}\mathbb{R^{k}}$. The Jacobian ${J(f)}$ is given by
% \begin{equation}
%     {{J_x({f})} = [\Delta_x{W_t^T[0]x}, \Delta_x{W_t^T[1]x}, \Delta_x{W_t^T[2]x}, ..., \Delta_x{W_t^T[\mathbb{K}]x}]}
% \end{equation}
% where as shown in Eq~\ref{eq:update} for the DPO training objective, 
% \begin{multline}
% \label{eq:jacob}
%     {W_t = W + \Sigma_{i=1}^p\alpha\gamma_ix_i[\mathbb{1},\mathbb{0,0,0,0},...] - \Sigma_{i=p+1}^t\alpha\gamma_ix_i[\mathbb{1},\mathbb{0,0,0,0},...]} - \\ {\Sigma_{i=1}^p\alpha\gamma_ix_i[\mathbb{0},\mathbb{1}(y_i==2),\mathbb{1}(y_i==3),..., \mathbb{1}(y_i==\mathbb{K})] +} \\ {\Sigma_{i=p+1}^t\alpha\gamma_ix_i[\mathbb{0},\mathbb{1}(y_i==2),\mathbb{1}(y_i==3),..., \mathbb{1}(y_i==\mathbb{K})]}
% \end{multline}

% For \bgdbox{green}{${x_i}$} $\sim$ \bgdbox{green}{$\mathcal{P_S}$}, 
% \begin{equation}
%      {\Delta_x{W_t^T[0]\bgdbox{green}{$x_i$}} = W^T[0] - \alpha\gamma_i\bgdbox{green}{$x_i$}}
% \end{equation}

% \begin{equation}
% {\Delta_x{W_t^T[j]\bgdbox{green}{$x_i$}} = W^T[j] + (\delta_i+\alpha\gamma_i)\gamma_i\bgdbox{green}{$x_i$}[\mathbb{1}(y_i==j)]}
% \end{equation}
% for ${j\neq 0}$

% For \bgdbox{red}{${x_k}$} $\sim$ \bgdbox{red}{$\mathcal{P_U}$}, 
% \begin{equation}
% {\Delta_x{W_t^T[0]\bgdbox{red}{$x_k$}} = W^T[0] + \alpha\gamma_k\bgdbox{red}{$x_k$}}
% \end{equation}

% \begin{equation}
% {\Delta_x{W_t^T[j]\bgdbox{red}{$x_k$}} = W^T[j] + (\delta_k-\alpha\gamma_k)\bgdbox{red}{$x_k$}[\mathbb{1}(y_k==j)]}
% \end{equation}
% for ${j\neq 0}$
% Thus for a safe sample \bgdbox{green}{${x_i}$} $\sim$ \bgdbox{green}{$\mathcal{P_S}$} belonging to class ${c}$,  $\mathbb{L_{{x_i}}({f_\theta^{DPO}})}$ is given by:
% \begin{multline}
%     \mathbb{L_{\bgdbox{green}{{$x_i$}}}(\mathtt{f_\theta^{DPO}})} = {||~~ (W^T[0] - \alpha\gamma_i\bgdbox{green}{$x_i$}), ~~ W^T[1], ~~W^T[2],~~ ..., ~~W^T[c] + (\delta_i+\alpha\gamma_i)\bgdbox{green}{$x_i$}\mathbb{1}(y_i==c)} \\ {~~, ...,~~ W^T[\mathbb{K}]~~||_{{p,q}}}
% \end{multline}
% Similarly for unsafe sample \bgdbox{red}{${x_i}$} $\sim$ \bgdbox{red}{$\mathcal{P_U}$}, the above expression is given by 
% \begin{multline}
%     \mathbb{L_{\bgdbox{red}{{$x_i$}}}({f_\theta^{DPO}})} = {||~~ (W^T[0] + \alpha\gamma_i\bgdbox{red}{$x_i$}), ~~ W^T[1], ~~W^T[2],~~ ..., ~~W^T[c] + (\delta_i-\alpha\gamma_i)\bgdbox{red}{$x_i$}\mathbb{1}(y_i==c)} \\ {~~, ...,~~ W^T[\mathbb{K}]~~||_{{p,q}}}
% \end{multline}



% Similarly, in case of unlearning, $\gamma_i$=1, which gives:
% \begin{multline}
% \label{eq:unlearn_unsafe_local}
%     \mathbb{L_{\bgdbox{red}{{$x_i$}}}({f_\theta^{Unl}})} = {||~~ (W^T[0] + \alpha\bgdbox{red}{$x_i$}), ~~ W^T[1], ~~W^T[2],~~ ..., ~~W^T[c] + (\delta_i-\alpha)\bgdbox{red}{$x_i$}\mathbb{1}(y_i==c)} \\ {~~, ...,~~ W^T[\mathbb{K}]~~||_{{p,q}}}
% \end{multline}


% \begin{multline}
%     \mathbb{L_{\bgdbox{green}{{$x_i$}}}({f_\theta^{Unl}})} = {||~~ (W^T[0] - \alpha\bgdbox{green}{$x_i$}), ~~ W^T[1], ~~W^T[2],~~ ..., ~~W^T[c] + (\delta_i+\alpha)\bgdbox{green}{$x_i$}\mathbb{1}(y_i==c)} \\ {~~, ...,~~ W^T[\mathbb{K}]~~||_{{p,q}}}
% \end{multline}




% Similarly, in case of SSFT, we will get:
% \begin{equation}
%     {L_{\bgdbox{red}{{$x_i$}}}({f_\theta^{SSFT}})} = {||~~ (W^T[0] + \alpha\bgdbox{red}{$x_i$}), ~~ W^T[1], ~~W^T[2],~~ ..., ~~W^T[c] + \delta_i\bgdbox{red}{$x_i$}\mathbb{1}(y_i==c)} \\ {~~, ...,~~ W^T[{k}]~~||_{{p,q}}}
% \end{equation}


% \begin{equation}
%     {L_{\bgdbox{green}{{$x_i$}}}({f_\theta^{SSFT}})} = {||~~ W^T[0], ~~ W^T[1], ~~W^T[2],~~ ..., ~~W^T[c] + (\delta_i+\alpha)\bgdbox{green}{$x_i$}\mathbb{1}(y_i==c)} \\ {~~, ...,~~ W^T[{k}]~~||_{{p,q}}}
% \end{equation}

% On the other hand, for the instruction fine-tuned model we have, $\alpha=0$, $\gamma=1$, thus we get:

% \begin{equation}
% \label{eq:IT_unsafe_local}
%     {L_{{{x_i}}}({f_\theta^{IT}})} = {||~~ W^T[0], ~~ W^T[1], ~~W^T[2],~~ ..., ~~W^T[c] + \delta_i{x_i}\mathbb{1}(y_i==c)} {~~, ...,~~ W^T[{k}]~~||_{{p,q}}}
% \end{equation}

% Since all the columns of weight matrix ${W}$ are orthogonal (since ${x_i^Tx_j=0, \forall i, j; i\neq j}$), on using the assumptions A4, A5 for ${p=q=2}$, we have
%  \begin{equation}
%  \label{eq:IT_spectral}
%  {||{L_{{{x_i}}}({f_\theta^{IT}})}||_{2,2} = ||W^T[c] + \delta_i{x_i}\mathbb{1}(y_i==c)||_2}
%  \end{equation}
 
% Whereas for unlearning, we get
% \begin{equation} 
% \label{eq:unlean_unsafe_spectral}
%  ||{L_{\bgdbox{red}{{$x_i$}}}({f_\theta^{Unl}})}||_{2,2} = {||W^T[c] + (\delta_i-\alpha)\bgdbox{red}{$x_i$}\mathbb{1}(y_i==c)||_2}
% \end{equation}

% \begin{equation}  
% \label{eq:unlean_safe_spectral}
%  ||{L_{\bgdbox{green}{{$x_i$}}}({f_\theta^{Unl}})}||_{2,2} = {||W^T[c] + (\delta_i+\alpha)\bgdbox{green}{$x_i$}\mathbb{1}(y_i==c)||_2}
% \end{equation}

%  Similarly for SSFT, we have
% \begin{equation} 
% \label{eq:SSFT_unsafe_spectral}
%  ||{L_{\bgdbox{red}{{$x_i$}}}({f_\theta^{SSFT}})}||_{2,2} = {||W^T[c] + \delta_i\bgdbox{red}{$x_i$}\mathbb{1}(y_i==c)||_2}
% \end{equation}

% \begin{equation}  
% \label{eq:SSFT_safe_spectral}
%  ||{L_{\bgdbox{green}{{$x_i$}}}({f_\theta^{SSFT}})}||_{2,2} = {||W^T[c] + (\delta_i+\alpha)\bgdbox{green}{$x_i$}\mathbb{1}(y_i==c)||_2}
% \end{equation}

% Comparing Eq~\ref{eq:unlean_unsafe_spectral}, \ref{eq:SSFT_unsafe_spectral} and \ref{eq:IT_spectral} for a given input ${x_i}$, we have $\exists$ $\alpha$, $\alpha\leq\delta_i$ such that

% $||{L_{\bgdbox{red}{{$x_i$}}}({f_\theta^{Unlr}})}||_{2,2} \leq ||{L_{\bgdbox{red}{{$x_i$}}}({f_\theta^{SSFT}})}||_{2,2} \approx ||{L_{{{x_i}}}({f_\theta^{IT}})}||_{2,2} $
% This also holds for DPO, but for the condition $\gamma_i\alpha\leq
% \delta_i$, thus $||{L_{\bgdbox{red}{{$x_i$}}}({f_\theta^{DPO}})}||_{2,2} \leq ||{L_{\bgdbox{red}{{$x_i$}}}({f_\theta^{SSFT}})}||_{2,2} \approx ||{L_{{{x_i}}}({f_\theta^{IT}})}||_{2,2} $
% This shows that the local lipschitzness of the model for unsafe samples should decrease on using unlearning and DPO, if appropriate learning rate is used.
% \end{proof}
